Advances and new ideas for neutron-capture astrophysics experiments at CERN n_TOF

This article presents a few selected developments and future ideas related to the measurement of $(n,\gamma)$ data of astrophysical interest at CERN n_TOF. The MC-aided analysis methodology for the use of low-efficiency radiation detectors in time-of-flight neutron-capture measurements is discussed, with particular emphasis on the systematic accuracy. Several recent instrumental advances are also presented, such as the development of total-energy detectors with $\gamma$-ray imaging capability for background suppression, and the development of an array of small-volume organic scintillators aimed at exploiting the high instantaneous neutron-flux of EAR2. Finally, astrophysics prospects related to the intermediate $i$ neutron-capture process of nucleosynthesis are discussed in the context of the new NEAR activation area.

==> repair.36767.csnameendcsname.tex <==
%% LaTeX2e file `csnameendcsname'
%% generated by the `filecontents' environment
%% from source `epj_FK' on 2022/08/03.
%%

